Influence Factors on RAG Poisoning

Retrieval-Augmented Generation (RAG) systems enhance large language models by grounding responses in retrieved documents from external knowledge sources at inference time. However, this reliance on retrieved content introduces vulnerabilities to poisoning attacks, in which adversarial documents can manipulate both the retrieval process and the generated outputs. This paper investigates poisoning robustness in RAG through a full factorial experimental study covering 432 configurations. We analyze the impacts of dataset, retriever type, retrieval depth, database composition, chunking strategy, and generator model on retrieval-level and generation-level metrics. The results show that retriever architecture, dataset, and retrieval depth are the strongest factors affecting poisoning exposure, while generator choice and database composition have a major impact on downstream attack success. Dense and graph-based retrievers generally improve robustness relative to BM25, whereas larger retrieval depth increases the likelihood of retrieving poisoned passages. We further show that replicating poisoned content across multiple databases amplifies adversarial influence, while additional clean sources can mitigate it. These findings highlight that poisoning vulnerability in RAG is not attributable to a single component, but instead arises from the interaction of retrieval, generation, and knowledge-base configuration.

==> sections/comments.tex <==
\subsection{Reviewer \#1}

\textbf{Comment \#1:} The paper should clarify more explicitly what is genuinely novel with respect to prior work, because the related work section already discusses many of the same factors, including retriever type, top-k, chunking, and generator dependence. As written, the contribution can appear more as a systematic comparison than as a clearly distinct research advance.

\textbf{Response \#1:} We thank the reviewer for this and all observations. To address this concern, we have revised the corresponding paragraph in the Introduction section to more explicitly articulate the novelty of the work. The updated text now highlights that unlike prior work that examines influence factors individually, this study conducts a full factorial experimental design that enables the quantification of compound and higher-order interaction effects among pipeline components. It also explicitly positions the number of databases and number of poisoned databases as novel experimental variables that have received comparatively little attention in prior work, enabling the study of adversarial redundancy and clean-source competition as distinct poisoning dimensions. These changes make the distinction between a systematic replication of known factors and a genuinely novel multi-factor interaction study explicit from the outset of the paper.

\begin{center}
\begin{minipage}{0.50\textwidth}
{\color{revieworange}\footnotesize
... Unlike prior work that examines such factors individually, we conduct a full factorial experimental study that enables the quantification of higher-order interaction effects among pipeline components. ... Crucially, we also introduce the number of databases and number of poisoned databases as experimental variables, a configuration dimension that has received little attention in prior work. ... This experimental design makes it possible to analyze not only whether poisoning succeeds, but also under which compound conditions it becomes more effective, more stealthy, or more damaging to answer quality. (page 2)
}
\end{minipage}
\end{center}


\textbf{Comment \#2:} The paper should discuss generalizability more carefully. Since the experiments rely on only two datasets, two generators, and a 100-pair curated subset, the conclusions should be framed more cautiously. The paper would benefit from a more explicit discussion of what can and cannot be generalized from this setup.

\textbf{Response \#2:} Since adding new experiments is not feasible at this stage, we revised the manuscript to clarify the scope of the conclusions. In the methodology, we now explain that the 100-pair subset was selected to obtain semantically similar questions between HotpotQA and MS MARCO, enabling a clearer controlled cross-dataset comparison, rather than representing the full distribution of either dataset. We also softened several claims throughout the results discussion by explicitly referring to the evaluated setup. Finally, we added a concise statement in the conclusion clarifying that the findings should be interpreted within the scope of the tested datasets, retrievers, generators, and curated subset, and we updated the future work paragraph to indicate that broader generalization requires larger and less curated query sets, additional datasets, more generator models, and more diverse poisoning attacks.

\begin{center}
\begin{minipage}{0.50\textwidth}
{\color{revieworange}\footnotesize
... This curated subset was chosen to enable a clearer cross-dataset comparison under aligned retrieval conditions, rather than to represent the full distribution of either dataset. ...
 (page 3)
\end{minipage}
\end{center}

\begin{center}
\begin{minipage}{0.50\textwidth}
{\color{revieworange}\footnotesize
Future work should extend this analysis to larger and less curated query sets, additional datasets and generator models, and a broader range of poisoning and retrieval-manipulation attacks, including more stealthy and adaptive attack strategies. (page 9)
\end{minipage}
\end{center}

\textbf{Comment \#3:} The paper should address reproducibility more clearly. For this kind of experimental study, it is important to state whether code, prompts, generated poisoned passages, and configuration scripts will be released. If they are not released, the authors should at least provide more implementation detail.

\textbf{Response \#3:} Due to the page limit constraints of the venue, we were unable to include full implementation details within the paper itself. However, to ensure reproducibility, we will make all experimental artifacts publicly available in a dedicated GitHub repository, upon paper acceptance. A reference to this repository will be added to the final version of the paper.
\\

\textbf{Comment \#4:} The paper would also be stronger if it connected its findings to concrete mitigation strategies. Since the results show that robustness depends on pipeline configuration, it would be useful to discuss defensive filtering methods that remove or down-rank adversarial passages before generation.

\textbf{Response \#4:} We have revised the discussion to better connect our findings to concrete mitigation strategies. In particular, we now emphasize that, since robustness depends on the retrieval and generation pipeline configuration, defenses should not only focus on the generator but also on the retrieved context before generation. We also added the suggested reference, ``Defending Against Knowledge Poisoning Attacks During Retrieval-Augmented Generation'' by Edemacu et al., because it is directly relevant to this point. 

\begin{center}
\begin{minipage}{0.50\textwidth}
{\color{revieworange}\footnotesize
These results motivate pre-generation mitigation strategies that filter or down-rank suspicious retrieved passages before they can influence the LLM output, aligning with recent work on defensive filtering against RAG poisoning \cite{edemacu}. (page 6)
\end{minipage}
\end{center}

\textbf{Comment \#5:} The authors could mention ``Defending Against Knowledge Poisoning Attacks During Retrieval-Augmented Generation'' by Edemacu et al., ``SafeRAG'' by Liang et al., and ``RevPRAG'' by Tan et al.


\textbf{Response \#5:} We thank the reviewer for these suggestions. SafeRAG (Liang et al.) is already included in our related work as reference [10], where we discuss how different LLMs vary in their susceptibility to poisoned evidence. We have also incorporated the work by Edemacu et al. on Comment 4. Due to page limitations, we were not able to include a detailed discussion of RevPRAG by Tan et al.; however, we recognize its relevance and have considered it as complementary work, particularly because it focuses on detecting poisoned responses through LLM activation analysis.
\\

\subsection{Reviewer \#2}

\textbf{Comment \#1:} Authors conclude that chunking (512 vs 768) has a ``limited influence''. However, this might be a result of your specific range. Differences between 128 and 1024 tokens might yield different results. You should frame this as ``within the tested parameters'' rather than a universal rule for RAG.

\textbf{Response \#1:} We thank the reviewer for this and all observations. We agree that substantially different ranges, such as 128 or 1024 tokens, may yield different dynamics. In Section 4, the chunking analysis paragraph scopes the conclusion to the tested parameter ranges, stating that \textit{``differences between the tested settings (512 vs. 768 tokens and overlaps of 64 vs. 100) produced no consistent or substantial changes''} and that \textit{``within the examined ranges, chunking configuration has a comparatively limited influence on poisoning exposure and downstream generation behavior when compared to factors such as retriever architecture, dataset choice, or retrieval depth''}.
\\

\textbf{Comment \#2:} The poisoning strategy relies on ``Target Claim + Question Overlap''. While this is a standard ``black-box'' attack, it doesn't account for Adversarial Embeddings (gradient-based attacks that hide poisoned documents in the vector space). Do your conclusions about ``Dense Retrieval Robustness'' hold up against attacks specifically designed to fool vector similarity.

\textbf{Response \#2:} We agree that our poisoning strategy does not cover adversarial embedding or gradient-based attacks designed specifically to manipulate vector similarity. Our attack is a black-box textual poisoning strategy based on target-claim insertion and question overlap, and therefore the conclusions about dense retrieval should be interpreted within this threat model. To clarify this, we revised the manuscript to state that the observed robustness of dense retrieval applies to the evaluated black-box attack and should not be generalized to adversarial embedding attacks. We also softened the discussion of dense retrieval robustness by referring to reduced exposure under the tested attack, rather than making a broad claim about dense retriever robustness in general.

\begin{center}
\begin{minipage}{0.50\textwidth}
{\color{revieworange}\footnotesize
Overall, within the evaluated  poisoning strategy, these findings suggest that semantic and structure-aware retrieval methods are less exposed to the tested adversarial passages than purely lexical retrieval approaches. (page 5)
\end{minipage}
\end{center}

\begin{center}
\begin{minipage}{0.50\textwidth}
{\color{revieworange}\footnotesize
In contrast, both the dense BGE and graph-based retrievers substantially reduce ASR under the evaluated attack, reinforcing that retrieval architecture is a key factor in this experimental setting. (page 6)
\end{minipage}
\end{center}

\begin{center}
\begin{minipage}{0.50\textwidth}
{\color{revieworange}\footnotesize
Future work should extend this analysis to larger and less curated query sets, additional datasets and generator models, and a broader range of poisoning and retrieval-manipulation attacks, including more stealthy and adaptive attack
strategies. (page 9)
\end{minipage}
\end{center}
\\

\textbf{Comment \#3:} Authors have to discuss why did HotpotQA exhibit larger Score Margins under graph retrieval compared to MS-MARCO? This seems to contradict the general trend of graph-based robustness.

\textbf{Response \#3:} The larger Score Margins observed on HotpotQA are a dataset-level main effect, independent of retriever type. The OLS regression (Table 1) shows that MS-MARCO dataset carries a coefficient of -0.114 on Score Margin, indicating that poisoned passages are less competitive on MS-MARCO across all retriever types, not exclusively under graph retrieval. The graph retriever maintains its own independent negative coefficient of -0.317 on Score Margin, confirming that it consistently reduces the competitiveness of poisoned passages relative to BM25 regardless of dataset. These two effects are additive, meaning that HotpotQA producing larger Score Margins overall does not diminish the protective contribution of graph retrieval within that dataset.






